Holography, Supergravity, and the Weak Gravity Conjecture

This dissertation represents work on three different subjects relating to quantum gravity and the AdS/CFT correspondence. First, we review a holographic computation of the one-loop corrections to the Weyl anomaly on Ricci flat backgrounds in six dimensions. This allows us to determine the correction to one linear combination of the anomaly coefficients. Then, we will show that these corrections may be obtained from the six-dimensional superconformal index. The second section covers consistent truncations on the Lunin-Maldacena background. We show how to restore minimal supersymmetry to this background by determining the reduction ansatz which includes the graviton and a gauge field of 5d $\mathcal{N} = 2$ supergravity. We also discuss our previously unpublished attempt to construct a truncation which includes a scalar field corresponding to the $\beta$-deformation parameter of the dual field theory. We show that if such a solution exists, it must differ drastically from the LM background. Finally, we discuss higher-derivative corrections to black hole solutions and the weak gravity conjecture in a few settings. First we compute higher-derivative corrections to the extremality bounds for black holes which are charged under an arbitrary number of $U(1)$ gauge fields, and determine the constraints implied by the WGC. Next we consider the higher-derivative corrections to thermodynamic quantities for charged black holes in Anti-de Sitter space. We confirm and clarify a previously noted relationship between the shift to the extremality bound and the shift to the Wald entropy. We also show that if the shift in the Wald entropy is assumed to be positive, then the coefficient of the $R_{\mu \nu \rho \sigma} R^{\mu \nu \rho \sigma}$ term in the effective Lagrangian must be positive as well.

==> Appendices/App3.tex <==
The bosonic matter content of type IIB supergravity consist of the NSNS fields $g_{\mu\nu}$, $B_{\mu\nu}$ and $\phi$ and the RR fields $\chi\equiv C_0$, $C_2$ and $C_4$.  The field strengths obtained from these potentials are defined by:
%
\begin{align}
    F_1 &= d \chi, \qquad  \qquad H_3 = d B_2, \qquad  \qquad F_3 = dC_2 \, - \chi H_3,\nn \\
    F_5 &= d C_4 - \frac{1}{2} \, ( \, C_2 \wedge \, H_3 \, - B_2 \, \wedge \, d C_2 \, ),
\end{align}
%
where $F_5$ is self-dual, $F_5=*F_5$.  The Bianchi identities then follow:
%
\begin{align}
    d F_1 &= 0, \qquad \qquad d F_3 - H_3 \wedge F_1 = 0,\nn \\
    d H_3 &= 0, \qquad \qquad d F_5 - H_3 \wedge F_3 = 0
\end{align}
%

Type IIB supergravity does not admit a covariant action because of the self-duality of $F_5$.  However, we can write down the equations of motion.  The form field equations are
%
\begin{align}
    d( e^{2 \phi} * F_1) &=- e^{\phi} H_3 \wedge * F_3,\nn\\
    d*d\phi &= e^{2 \phi} F_1 \wedge * F_1 - \ft12 e^{- \phi} H_3 \wedge * H_3+\ft12 e^{\phi} F_3 \wedge * F_3,\nn \\
    d( e^{- \phi} * H_3) &=e^{\phi} F_1 \wedge * F_3 +F_3 \wedge F_5,\nn\\
    d( e^{\phi} * F_3) &=-H_3 \wedge F_5,
\end{align}
%
and the Einstein equation in Ricci form is
%%%%
\begin{align}
    R_{\mu\nu}&=\fft12\partial_\mu\phi\partial_\nu\phi+\fft12e^{2\phi}\partial_\mu\chi\partial_\nu\chi+\fft14e^{-\phi}\left(H_{\mu\rho\sigma}H_\nu{}^{\rho\sigma}-\fft1{12}g_{\mu\nu}H_{\lambda\rho\sigma}H^{\lambda\rho\sigma}\right)\nn\\
    &\qquad+\fft14e^\phi\left(F_{\mu\rho\sigma}F_\nu{}^{\rho\sigma}-\fft1{12}g_{\mu\nu}F_{\lambda\rho\sigma}F^{\lambda\rho\sigma}\right)+\fft1{4\cdot4!}F_{\mu\lambda\rho\sigma\tau}F_\nu{}^{\lambda\rho\sigma\tau}.
\end{align}
%%%%

The above equations can reexpressed in terms of the complex fields
%
\begin{equation}
    \tau=\chi+ie^{-\phi},\qquad G_3=F_3-ie^{-\phi}H_3.
\end{equation}
%
In particular, we have
%
\begin{align}
    \fft{d*d\tau}{\tau_2}+i\fft{d\tau\wedge*d\tau}{\tau_2^2}&=-\fft{i}{2\tau_2}G_3\wedge*G_3,\nn\\
    d*G_3&=-i\fft{d\tau}{\tau_2}\wedge*\Re G_3+iF_5\wedge G_3,\nn\\
    dF_5&=\fft{i}{2\tau_2}G_3\wedge \overline{G}_3,
\end{align}
%
along with
%
\begin{equation}
    R_{\mu\nu}=\fft1{2\tau_2^2}\partial_{(\mu}\tau\partial_{\nu)}\bar\tau+\fft14\left(G_{(\mu}{}^{\rho\sigma}\overline{G}_{\nu)\rho\sigma}-\fft1{12}g_{\mu\nu}G_{\lambda\rho\sigma}\overline{G}^{\lambda\rho\sigma}\right)+\fft1{4\cdot4!}F_{\mu\lambda\rho\sigma\tau}F_\nu{}^{\lambda\rho\sigma\tau}.
\end{equation}
%
Here the overlines indicate complex conjugation.

==> Appendices/App9.tex <==
\noindent Recent work \cite{Cheung:2018cwt, Goon:2019faz} suggests a remarkable universal relationship between the corrections to extremality and corrections to entropy. Here we will present a simple derivation of this relation using standard thermodynamic identities, including a slight generalization of the relation away from extremality. The statement itself is not specific to black holes, and is in fact a relatively universal statement about infinitesimal deformations of thermodynamic systems.  

Consider a thermodynamic system, let $E$ be the total thermal energy, $T$ the temperature, $S$ the entropy and $X$ collectively label a set of extensive thermodynamic variables (for black holes this could be the charge $Q$ and spin $J$). Now consider a small deformation of this system parametrized by a continuous parameter $\epsilon$. The only assumption we will make about this deformation is that it preserves the third law of thermodynamics in the form
\begin{equation}\label{third}
  \lim_{T\rightarrow 0}TS(T,X,\epsilon) = 0,
\end{equation}
%
for all $\epsilon$ on an open neighbourhood of $\epsilon=0$.

We begin with the first law of thermodynamics in the form
\begin{equation}\label{first}
  1 = T\left(\frac{\partial S}{\partial E}\right)_{X,\epsilon}.
\end{equation}
%
Making use of the triple product identity
\begin{equation}
  \left(\frac{\partial S}{\partial E}\right)_{X,\epsilon}\left(\frac{\partial E}{\partial \epsilon}\right)_{X,S}\left(\frac{\partial \epsilon}{\partial S}\right)_{X,E} = -1,
\end{equation}
%
we have 
\begin{equation}
  \left(\frac{\partial E}{\partial \epsilon}\right)_{X,S} = -T \left(\frac{\partial S}{\partial \epsilon}\right)_{X,E}.
\end{equation}
%
Formally inverting $S(T,X,\epsilon)$ gives $T(S,X,\epsilon)$. We can use this to write 
\begin{equation}
   \left(\frac{\partial E}{\partial \epsilon}\right)_{X,S} =  \left(\frac{\partial E}{\partial \epsilon}\right)_{X,T} +  \left(\frac{\partial E}{\partial T}\right)_{X,\epsilon} \left(\frac{\partial T}{\partial \epsilon}\right)_{X,S}.
\end{equation}
%
Combining these
\begin{equation}
  \left(\frac{\partial E}{\partial \epsilon}\right)_{X,T} = -T \left(\frac{\partial S}{\partial \epsilon}\right)_{X,E} - \left(\frac{\partial E}{\partial T}\right)_{X,\epsilon} \left(\frac{\partial T}{\partial \epsilon}\right)_{X,S}.
\end{equation}
Next, we use (\ref{first}) again
\begin{align}
  \left(\frac{\partial E}{\partial \epsilon}\right)_{X,T} &= -T \left(\frac{\partial S}{\partial \epsilon}\right)_{X,E} - \left(\frac{\partial E}{\partial T}\right)_{X,\epsilon} \left(\frac{\partial T}{\partial \epsilon}\right)_{X,S} \nonumber\\
                                                          &=-T \left(\frac{\partial S}{\partial \epsilon}\right)_{X,E} - T\left(\frac{\partial S}{\partial E}\right)_{X,\epsilon}\left(\frac{\partial E}{\partial T}\right)_{X,\epsilon} \left(\frac{\partial T}{\partial \epsilon}\right)_{X,S} \nonumber\\
                                                          &=-T \left(\frac{\partial S}{\partial \epsilon}\right)_{X,E} - T\left(\frac{\partial S}{\partial T}\right)_{X,\epsilon} \left(\frac{\partial T}{\partial \epsilon}\right)_{X,S},
\end{align}
%
one final application of the triple product identity gives the \textit{generalized Goon-Penco relation}
%
\begin{equation}\label{result}
   \left(\frac{\partial E}{\partial \epsilon}\right)_{X,T} +T \left(\frac{\partial S}{\partial \epsilon}\right)_{X,E} = T \left(\frac{\partial S}{\partial \epsilon}\right)_{X,T}.
\end{equation}
%
Next we make use of the assumption that the deformation does not violate the third law of thermodynamics. Taylor expanding (\ref{first}) we have
\begin{equation}
  \lim_{T\rightarrow 0} \left[TS(T,X,\epsilon=0) + \epsilon T \left(\frac{\partial S}{\partial \epsilon}\right)_{T,X}\biggr\vert_{\epsilon=0} +\mathcal{O}\left(\epsilon^2\right)\right] = 0.
\end{equation}
%
By assumption this is true on an open neighbourhood of $\epsilon=0$ and so must be true order-by-order in the expansion, this gives
\begin{equation}
  \lim_{T\rightarrow 0} T\left(\frac{\partial S}{\partial \epsilon}\right)_{T,X}\biggr\vert_{\epsilon=0} = 0 \, .
\end{equation}
%
Using this together with (\ref{result}) gives the Goon-Penco relation
%
\begin{equation}
      \boxed{\lim_{T\rightarrow 0}\left[\left(\frac{\partial E}{\partial \epsilon}\right)_{X,T}\biggr\vert_{\epsilon=0} +T \left(\frac{\partial S}{\partial \epsilon}\right)_{X,E}\biggr\vert_{\epsilon=0}\right] = 0.}
\end{equation}
%
For the specific application to black hole thermodynamics we identify $E$ with the mass $M$ of the black hole, $X$ with the black hole parameters measured at infinity such as charge $Q$ or angular momentum $J$, and $\epsilon$ with a Wilson coefficient of a four-derivative effective operator. 

In section III, we have pointed out that shift in charge at fixed mass is also proportional to the entropy shift and mass shift. This statement can be derived similarly. By the triple product identity, 
%
\begin{align}
\begin{split}
    \left( \frac{\partial E}{\partial \epsilon} \right)_{X_i, T} = - \left( \frac{\partial X_i}{\partial \epsilon} \right)_{E, T} \left( \frac{\partial E}{\partial X_i} \right)_{\epsilon, T} \, .
\end{split}
\end{align}
%
This holds for any extensive quantity. Now we choose $X_i = Q$, and we may identify 
%
\begin{align}
    \left( \frac{\partial E}{\partial X_i} \right)_{\epsilon, T} = \Phi.
\end{align}
%
So we find 
%
\begin{align}
\begin{split}
    \left( \frac{\partial E}{\partial \epsilon} \right)_{Q, T} =  -\Phi \left( \frac{\partial Q}{\partial \epsilon} \right)_{E, T}.
\end{split}
\end{align}
%
For black holes, this means that the shift in charge is related to the shift in mass.  Neither of them is related to the entropy except at extremality. The result of this is that the entropy shift at extremality may be related to the extremality shift at constant charge or at constant mass,
%
\begin{align}
    \lim_{T\rightarrow 0} \left( \frac{\partial E}{\partial \epsilon} \right)_{Q, T} = - \lim_{T\rightarrow 0}  \Phi \left( \frac{\partial Q}{\partial \epsilon} \right)_{E, T} =  - \lim_{T\rightarrow 0} T \left(\frac{\partial S}{\partial \epsilon}\right)_{Q,E}.
\end{align}

\section{Comment on $\alpha'$-Corrections to Black Holes in Heterotic String Theory }

\noindent Recent work has considered the leading $\alpha'$-corrections to dyonic Reissner-Nordstr{\"o}m black holes embedded in heterotic string theory \cite{Cano:2019oma, Cano:2019ycn}. Though the four-dimensional backgrounds considered in these papers are asymptotically flat, we would like to briefly comment on them in connection with the universal entropy-extremality relationship.

From the dimensionally reduced, effective four-dimensional solutions the authors calculated explicit expressions for the Wald entropy, 
\begin{equation}
   S =  \pi  \left[\left(\mu +M\right)^2+\epsilon  \alpha ' \frac{\left(18 M \mu+21
   \mu^2 +M^2\right)}{40 \mu
   \left(\mu+M\right)}
   \right],
\end{equation}
%
and Hawking temperature,
\begin{equation} \label{alphaT}
    T =\frac{\mu}{2 \pi
    \left(\mu + M \right)^2}+\epsilon  \alpha '\frac{ \left(M + 3 \mu \right)
   \left( M-\mu \right)^2}{160 \pi  \mu
   \left(\mu +M \right)^5},
\end{equation}
%
where we have defined $\mu = \sqrt{M^2-\frac{P^2}{2}}$. Here $P$ denotes the charge of the black hole, and we have adopted the same small expansion parameter $\epsilon$ as earlier. From these results it is straightforward to verify the following relation 
\begin{equation}
    T^{-1} = \left(\frac{\partial S}{ \partial M}\right)_P,
\end{equation}
%
up to errors of $\mathcal{O}(\epsilon^2)$. Consequently, the parameter $M$ corresponds to the thermal mass of the black hole. With these explicit expressions we can verify the entropy-extremality relation derived in \cite{Goon:2019faz}. The differential change in the mass at fixed temperature is given by a simple application of the triple product identity,
\begin{equation} \label{alphaDM}
   \left(\frac{\partial M}{\partial \epsilon}\right)_{T,P} = -\frac{\left(\frac{\partial T}{\partial \epsilon}\right)_{M,P}}{\left(\frac{\partial T}{\partial M}\right)_{\epsilon,P}}\biggr\vert_{\epsilon=0}.
\end{equation}
%
The differential change in the \textit{extremal} mass is given by taking $T\rightarrow 0^+$. This limit must be taken indirectly since the function (\ref{alphaT}) is too complicated to be inverted directly. The zero temperature limit is then the same as taking $M\rightarrow M_{\text{ext}}$. Since (\ref{alphaDM}) is already a relation between two quantities at $\mathcal{O}(\alpha')$, we only require  $M\rightarrow (M_{\text{ext}})_0$, which is the leading-order extremality relationship
\begin{equation}
    (M_{\text{ext}})_0 = \frac{|P|}{\sqrt{2}}.
\end{equation}
%
The correction to the extremal mass is then found to be
\begin{equation}
    \left(\frac{\partial M}{\partial \epsilon}\right)_{T = 0,P} = -\frac{\alpha'}{40\sqrt{2}|P|},
    \label{cano_mass}
\end{equation}
%
in agreement with \cite{Cano:2019ycn}.
To verify the entropy-extremality relation we also need the shift to the entropy at fixed charge and mass. Since the Wald entropy given above is already parametrized in terms of the thermal mass and charge, this is trivial to calculate,
\begin{equation}
    \left(\frac{\partial S}{\partial \epsilon}\right)_{M,P} =   \alpha '\pi \frac{\left(M^2 + 18 M \mu +21
   \mu^2 \right)}{40 \mu
   \left(\mu +M\right)}.
\end{equation}
%
According to \cite{Goon:2019faz}, we should take the zero temperature limit of this expression multiplied by the uncorrected temperature. This is equivalent to taking $M\rightarrow (M_{\text{ext}})_0$. 
Indeed, taking this limit we find
\begin{equation}
\label{T0DeltaS}
    \lim_{T\rightarrow 0} T_0 \left(\frac{\partial S}{\partial \epsilon}\right)_{M,P} = \lim_{M\rightarrow (M_{\text{ext}})_0} \;\lim_{\epsilon \rightarrow 0} \;T(M,P,\epsilon) \left(\frac{\partial S}{\partial \epsilon}\right)_{M,P} = \frac{\alpha'}{40\sqrt{2}|P|}\, ,
\end{equation}
%
which agrees precisely with the shift to the mass in (\ref{cano_mass}), verifying the entropy-extremality relationship.  
While (\ref{T0DeltaS}) was also reproduced in \cite{Cano:2019ycn}, the authors suggest that it may be more convenient to work in a near-extremal regime, in which the result of \cite{Goon:2019faz}
would be modified.
In particular, in the ``very near-extremal" regime  discussed in \cite{Cano:2019ycn}, in which one extracts the leading order terms in the near extremal temperature and near extremal entropy (both contributions of order $\sqrt{\epsilon}$), one
finds 
$\frac{\alpha'}{80\sqrt{2}|P|}$,
which differs from
(\ref{T0DeltaS}) precisely by a factor of $1/2$.

Such issues are related to the claim 
of \cite{Cano:2019ycn} that the positivity of the 
entropy shift 
doesn't necessarily imply a positive correction 
to the charge to mass ratio at extremality.
%
Here we would like to further clarify the 
validity of the results of \cite{Goon:2019faz}, 
and stress that the order of limits 
was \emph{crucial} in order to obtain (\ref{T0DeltaS}).
Indeed, if the limits were taken in 
the other order, we would find
\begin{equation}
    \lim_{\epsilon \rightarrow 0}\;\lim_{M\rightarrow M_{\text{ext}}}  \;T(M,P,\epsilon) \left(\frac{\partial S}{\partial \epsilon}\right)_{M,P} = \frac{\alpha'}{60\sqrt{2}|P|},
\end{equation}
%
which does not agree with the correction to the extremal mass. The near-extremal computation that yields the $1/2$ factor mentioned above is yet another way to compute $T \Delta S$, which not surprisingly leads to a different value. The final result is indeed extremely sensitive to the
way in which one approaches extremality. 
%
Nonetheless, the results of \cite{Goon:2019faz} are valid in general,  provided the extremality limit is taken in a  precise way, as described by (\ref{T0DeltaS}).

==> Chap2/misc.tex <==
Studying quantum field theories at large coupling is one of the most challenging and important problems in theoretical physics. Superconformal field theories are a restricted class where we may obtain a number of answers which are not available for general quantum field theories. This is because the rich symmetry structure of these theories allows for special tools to study them. In particular, the AdS/CFT correspondence and supersymmetric localization have led to a number of insights into the structure of these theories. First we will review some of the basic features of superconformal field theories.

The basic symmetries of flat space include translations, rotations, and boosts. This symmetry group is generated by the Poincar\'e Algebra, whose commutation relations are 
%
\begin{align}
    \begin{split}
        [M_{\mu \nu}, P_{\rho}] &= i(\eta_{\mu \rho}P_{\nu} - \eta_{\nu \rho}P_{\mu})\\  
        [M_{\mu \nu}, M_{\rho \sigma}] &= i( \eta_{\mu \rho} M_{\nu \sigma} -\eta_{\mu \sigma} M_{\nu \rho} -\eta_{\nu \rho} M_{\mu \sigma}+ \eta_{\nu \sigma}M_{\mu \rho}) \,
    \end{split}
\end{align}
%
where $P$ generate translations and $M$ the rotations and boosts. For superconformal field theories, the group of spacetime symmetries is enlarged by adding (1) scale transformations $D$ and special conformal transformations $K_{\mu}$, which together generate the conformal group,
%
\begin{align}
\begin{split}
        [D, K_{\mu}] &= -i K_{\mu}\\
        [D, P_{\mu}] &= i P_{\mu}\\
        [K_{\mu}, P_{\nu}] &= 2i(\eta_{\mu \nu} D - M_{\mu \nu}) \\
        [M_{\mu \nu}, K_{\rho}] &= i(\eta_{\mu \rho}K_{\nu} - \eta_{\nu \rho}K_{\mu})
\end{split}
\end{align}
%
(2) fermionic generators of supersymmetry transformations $Q$ and $S$,
%
\begin{align}
    \{ Q_a \, , \, \bar{Q}_{\dot{b}} \} \ = \ 2 \sigma^{\mu}_{a \dot{b}} P^\mu \\ 
    \{ S_a \, , \, \bar{S}_{\dot{b}} \} \ = \ 2 \sigma^{\mu}_{a \dot{b}} K^\mu 
\end{align}
and (3) generators of $R$-symmetry $T$, which act on the SUSY generators, and whose form depends on the amount of supersymmetry
%
There are a number of other commutation relations which we did not write, many of which are zero.

==> abbr.tex <==
\acro{CFT}{conformal field theory}
\acro{AdS}{Anti-de Sitter space}
\acro{EFT}{effective field theory}
\acro{WGC}{weak gravity conjecture}
\acro{AdS-RN}{Anti-de Sitter Riessner-Nordstr{\"o}m}
\acro{LM}{Lunin-Maldacena}
\acro{GR}{General Relativity}
\acro{KK}{Kaluza-Klein}
